$L^*LM$: Learning Automata from Examples using Natural Language Oracles

Expert demonstrations have proven an easy way to indirectly specify complex tasks. Recent algorithms even support extracting unambiguous formal specifications, e.g. deterministic finite automata (DFA), from demonstrations. Unfortunately, these techniques are generally not sample efficient. In this work, we introduce $L^*LM$, an algorithm for learning DFAs from both demonstrations and natural language. Due to the expressivity of natural language, we observe a significant improvement in the data efficiency of learning DFAs from expert demonstrations. Technically, $L^*LM$ leverages large language models to answer membership queries about the underlying task. This is then combined with recent techniques for transforming learning from demonstrations into a sequence of labeled example learning problems. In our experiments, we observe the two modalities complement each other, yielding a powerful few-shot learner.

==> interaction.tex <==
\paragraph{LLM interaction using direct yes/no/unsure\\}
\label{sec:llm_oracle_interaction}
Generated using ChatGPT-4o:
\\

\begin{lstlisting}[frame=single, basicstyle=\ttfamily, framexleftmargin=10pt, xleftmargin=20pt]
A robot is operating in a grid world and can visit four types of tiles: {red, yellow, blue, green}.

They correspond to lava (red), recharging (yellow), water (blue), and drying (green) tiles.

The robot is to visit tiles according to some set of rules. This will be recorded as a sequence of colors.

Rules include:

    1. The sequence must contain at least one yellow tile, i.e., eventually recharge. 
    2. The sequence must not contain any red tiles, i.e., lava must be avoided at all costs.
    3. If blue is visited, then you must visit green *before* yellow, i.e., the robot must dry off before recharging.

A positive example must conform to all rules.

Further note that repeated sequential colors can be replaced with a single
instance.

For example:
 - [yellow,yellow,blue] => [yellow, blue]
 - [red,red,blue,green,green,red] => [red,blue,green,red]
 - [blue,blue,blue] => [blue]

Additionally, by examining demonstrations of the task, we conjecture the following labeled examples:

POSITIVE EXAMPLES
  - [blue, green, yellow]
  - [yellow]

NEGATIVE EXAMPLES
  - [blue, red, yellow]
  - [red, yellow, green]
  - [blue, red, blue, red]
  - [blue]
  - [blue, red, green, yellow]
  - [blue, green]
  - [blue, yellow]

Please briefly answer the following questions using step-by-step reasoning to show your work. Do not answer any other question. When you arrive at a conclusion, please state it as FINAL_ANSWER: <yes, no>.

\end{lstlisting}

\begin{lstlisting}[frame=none, basicstyle=\ttfamily, framexleftmargin=10pt, xleftmargin=20pt]
User: Is [red, red, blue] a positive example?

AI: To determine if [red, red, blue] is a positive example, we need to check if it conforms to all the rules.

1) The sequence must contain at least one yellow tile - FINAL_ANSWER: no

User: Is [yellow, blue] a positive example? 

AI: To determine if [yellow, blue] is a positive example, we need to check if it conforms to all the rules. 

1) The sequence must contain at least one yellow tile - FINAL_ANSWER: yes 


User: Is [red, blue] a positive example?

AI: To determine if [red, blue] is a positive example, we need to check if it
conforms to all the rules. 

1) The sequence must not contain any red tiles - FINAL_ANSWER: no


User: Is [yellow, yellow, green] a positive example?

AI: To determine if [yellow, yellow, green] is a positive example, we need to
check if it conforms to all the rules. 

1) The sequence must contain at least one yellow tile - FINAL_ANSWER: yes


User: Is [yellow, blue, blue] a positive example?

AI: To determine if [yellow, blue, blue] is a positive example, we need to
check if it conforms to all the rules. 

1) The sequence must not contain any red tiles - FINAL_ANSWER: yes


User: Is [yellow, yellow] a positive example?

AI: To determine if [yellow, yellow] is a positive example, we need to check if
it conforms to all the rules. 

1) The sequence must contain at least one yellow tile - FINAL_ANSWER: yes


User: Is [yellow, red, green, yellow] a positive example?

AI: To determine if [yellow, red, green, yellow] is a positive example, we need to check if it conforms to all the rules. 

1) The sequence must not contain any red tiles - FINAL_ANSWER: no

\end{lstlisting}

\clearpage

\subsection{LLM interaction generating code to answer yes/no/unsure}
The following was generated from ChatGPT-4o. Our prompt:

\begin{lstlisting}[frame=single, basicstyle=\ttfamily, framexleftmargin=10pt, xleftmargin=20pt]
A robot is operating in a grid world and can visit four types of tiles: {red, yellow, blue, green}.

They correspond to lava (red), recharging (yellow), water (blue), and drying (green) tiles.

The robot is to visit tiles according to some set of rules. This will be recorded as a sequence of colors.

Rules include:

    1. The sequence must contain at least one yellow tile, i.e., eventually recharge. 
    2. The sequence must not contain any red tiles, i.e., lava must be avoided at all costs.

A positive example must conform to all rules.

Further note that repeated sequential colors can be replaced with a single instance.

For example:
 - [yellow,yellow,blue] => [yellow, blue]
 - [red,red,blue,green,green,red] => [red,blue,green,red]
 - [blue,blue,blue] => [blue]


Additionally, by examining demonstrations of the task, we conjecture the following labeled examples:


POSITIVE EXAMPLES
  - [blue, green, yellow]
  - [yellow]

NEGATIVE EXAMPLES
  - [blue, red, yellow]
  - [red, yellow, green]
  - [blue, red, blue, red]
  - [blue]
  - [blue, red, green, yellow]
  - [blue, green]
  - [blue, yellow]


Using step-by-step reasoning to create a python program to encode the above rules. Show your work. Do not answer any other question. The input of the python program will be a list of colors and the output should be "yes", "no", or "unsure".

\end{lstlisting}

\noindent
GPT-4o's response:
\begin{lstlisting}[frame=none, basicstyle=\ttfamily, framexleftmargin=10pt, xleftmargin=20pt]
To create a Python program that follows the rules and checks whether a sequence of tiles is a valid path according to the given conditions, we need to systematically break down the requirements and encode them step-by-step.

Here's a step-by-step explanation of the logic we'll implement:

    Deduplicate Sequential Colors: If the same color appears consecutively, we will reduce them to a single instance of that color.

    Check for Rules:
        The sequence must contain at least one yellow tile.
        The sequence must not contain any red tiles.

    Determine Positive or Negative Example:
        If the sequence contains "red", it's an immediate "no".
        If the sequence does not contain any "yellow", it's an immediate "no".
        If the sequence meets the above criteria but does not conform to the known
        patterns of positive or negative examples, it will be labeled as "unsure".

Here is the Python code to achieve this:

\end{lstlisting}

\noindent
\texttt{python}
\begin{lstlisting}[language=Python]
def deduplicate_sequence(sequence):
  """Remove consecutive duplicates from the sequence."""
  if not sequence:
    return []
  deduplicated = [sequence[0]]
  for color in sequence[1:]:
    if color != deduplicated[-1]:
      deduplicated.append(color)
  return deduplicated

def is_valid_sequence(sequence):
  """Check if the sequence is valid based on the given rules."""
  deduplicated = deduplicate_sequence(sequence)

  # Check for red tiles
  if "red" in deduplicated:
    return "no"

  # Check for at least one yellow tile
  if "yellow" not in deduplicated:
    return "no"

  # Compare against positive examples
  positive_examples = [
    ["blue", "green", "yellow"],
    ["yellow"]
  ]
  if deduplicated in positive_examples:
    return "yes"

  # Compare against negative examples
  negative_examples = [
    ["blue", "red", "yellow"],
    ["red", "yellow", "green"],
    ["blue", "red", "blue", "red"],
    ["blue"],
    ["blue", "red", "green", "yellow"],
    ["blue", "green"],
    ["blue", "yellow"]
  ]
  if deduplicated in negative_examples:
    return "no"

  # If it doesn't match any known patterns, return "unsure"
    return "unsure"

\end{lstlisting}

\clearpage

\subsection{LLM interaction generating code to answer yes/no}\label{sec:llm_code_oracle}
The following was generated from ChatGPT-4o. Our prompt:

\begin{lstlisting}[frame=single, basicstyle=\ttfamily, framexleftmargin=10pt, xleftmargin=20pt]
A robot is operating in a grid world and can visit four types of tiles: {red, yellow, blue, green}.

They correspond to lava (red), recharging (yellow), water (blue), and drying (green) tiles.

The robot is to visit tiles according to some set of rules. This will be recorded as a sequence of colors.

Rules include:

    1. The sequence must contain at least one yellow tile, i.e., eventually recharge. 
    2. The sequence must not contain any red tiles, i.e., lava must be avoided at all costs.

A positive example must conform to all rules.

Further note that repeated sequential colors can be replaced with a single instance.

For example:
 - [yellow,yellow,blue] => [yellow, blue]
 - [red,red,blue,green,green,red] => [red,blue,green,red]
 - [blue,blue,blue] => [blue]


Additionally, by examining demonstrations of the task, we conjecture the following labeled examples:


POSITIVE EXAMPLES
  - [blue, green, yellow]
  - [yellow]

NEGATIVE EXAMPLES
  - [blue, red, yellow]
  - [red, yellow, green]
  - [blue, red, blue, red]
  - [blue]
  - [blue, red, green, yellow]
  - [blue, green]
  - [blue, yellow]

Using step-by-step reasoning to create a python program to encode the above rules. Show your work. Do not answer any other question. The input of the python program will be a list of colors and the output should be "yes", "no".

\end{lstlisting}

\noindent
ChatGPT:
\begin{lstlisting}[frame=none, basicstyle=\ttfamily, framexleftmargin=10pt, xleftmargin=20pt]
To create a Python program that checks if a given sequence of tiles meets the specified rules, let's break down the steps needed:

    Check for at least one yellow tile: The sequence must contain at least one yellow tile.
    Check for the absence of red tiles: The sequence must not contain any red tiles.
    Simplify the sequence: Remove consecutive repeated colors to simplify the sequence.

Here's a step-by-step breakdown of the code:

    Define the function: The function will take a list of colors as input and return "yes" or "no" based on whether the sequence meets the rules.

    Simplify the sequence: Remove consecutive duplicates.

    Check for at least one yellow tile: Ensure there is at least one yellow tile in the simplified sequence.

    Check for absence of red tiles: Ensure there are no red tiles in the simplified sequence.

Here's the Python program that accomplishes this:

\end{lstlisting}

\noindent
\texttt{python}
\begin{lstlisting}[language=Python]
def check_sequence(sequence):
  # Step 1: Simplify the sequence to remove consecutive duplicates
  simplified_sequence = []
  for color in sequence:
    if not simplified_sequence or simplified_sequence[-1] != color:
      simplified_sequence.append(color)

  # Step 2: Check for at least one yellow tile
  if 'yellow' not in simplified_sequence:
    return "no"

  # Step 3: Check for absence of red tiles
  if 'red' in simplified_sequence:
    return "no"

  # If all checks are passed
  return "yes" 

\end{lstlisting}


==> task_prompt.tex <==
\begin{verbatim}
A robot is operating in a grid world and can visit four types of tiles:
{red, yellow, blue, green}.
They correspond to lava (red), recharging (yellow), water (blue), 
and drying (green) tiles.
The robot is to visit tiles according to some set of rules. This will be recorded as a
sequence of colors.

Rules include:

1. The sequence must contain at least one yellow tile, i.e., eventually recharge. 
2. The sequence must not contain any red tiles, i.e., lava must be avoided 
   at all costs.
3. If blue is visited, then you must visit green *before* yellow, i.e., the robot 
   must dry off before recharging.


A positive example must conform to all rules.
Further note that repeated sequential colors can be replaced with a single instance.

For example:
1. [yellow,yellow,blue] => [yellow, blue]
2. [red,red,blue,green,green,red] => [red,blue,green,red]
3. [blue,blue,blue] => [blue]
\end{verbatim}

